Harnessing Correlations in Distributed Erasure-Coded Key-Value Stores

Motivated by applications of distributed storage systems to key-value stores, the multi-version coding problem was formulated to efficiently store frequently updated data in asynchronous decentralized storage systems. Inspired by consistency requirements in distributed systems, the main goal in the multi-version coding problem is to ensure that the latest possible version of the data is decodable, even if the data updates have not reached some servers in the system. In this paper, we study the storage cost of ensuring consistency for the case where the data versions are correlated, in contrast to previous work where data versions were treated as being independent. We provide multi-version code constructions that show that the storage cost can be significantly smaller than the previous constructions depending on the degree of correlation, despite the asynchrony and the decentralized nature. Our achievability results are based on Reed-Solomon codes and random binning. Through an information-theoretic converse, we show that our multi-version codes are nearly-optimal, within a factor of $2$, in certain interesting regimes.

==> lowerbound_stronger.tex <==
\section{Lower Bound on The Storage Cost}
\label{Lower Bound on the storage cost}
In this section, we derive a lower bound based on the idea of \cite{multi_arxiv} for the case where we have correlated versions, and we require successful decoding with probability that is at least $1-\epsilon_K$. It was noted in \cite{multi_arxiv} that, for the case where $W_1 \rightarrow W_2 \rightarrow \ldots W_{\nu},$ where $W_{i}$ are Bernoulli $1/2$ vectors, with $W_{i}\in\{0,1\}^{K}$ is derived in an i.i.d. manner with flipping each bit of $W_{i-1}$ with probability $p,$ the storage cost of a multi-version code is $\frac{H(W_1,W_2,\ldots,W_{\nu})}{\nu+c-1} = \frac{K}{c+v-1} + \frac{(\nu-1) H(p)}{\nu+c-1}.$ We note that the remark of \cite{multi_arxiv} is applicable when $\delta_K=p,$ that is $\delta_K$ is constant - this is because the usual law of large numbers implies that in both the i.i.d. case and for the case where $\delta_K$ is a constant, most of the sequences of $W_{i}$ are concentrated in small spherical shell of radius $p$ around $W_{i-1}$. We are interested in the more general case where $\delta_{K}$ is not necessarily a constant. The ideas of \cite{multi_arxiv} can be extended to this more general case to show a lower bound of  $\frac{K}{c+v-1}+\frac{(\nu-1)\log Vol(\delta_K K)}{c+\nu-1}$. For the case of $\delta_K=o(K)$, note that there is a large gap between this lower bound and our achievable schemes; specifically, all our achievable schemes have a storage cost of $\frac{K}{c}+o(K)$ whereas the lower bound has a storage cost of $\frac{K}{c+\nu-1} + o(K)$. 

Since our goal is to evaluate the effectiveness of the scheme of Theorem \ref{}, we will develop a new lower bound of the form $\frac{K}{c}+\lambda \log Vol(\delta_K K) + o(\log Vol(\delta_K K)),$ where $\lambda$ is a constant. Once we obtain such a bound, the second order term in the lower bound $\lambda$ can be compared with the second order terms of the coding schemes presented in previous sections.

To keep our exposition clear, we will simply present the proof for $\nu=2$. The 


We begin with some lemmas. Recall that a ball in the Hamming space is a set of the form $\mathcal{B}(\vec{v},r)$. 

\begin{lemma}[Gilbert-Varshamov Bound]
The set $\{0,1\}^{K}$ consists of at least $\frac{2^{K}}{\log(Vol(K,2r))}$ disjoint balls of radius $r$. 
\end{lemma}

\begin{lemma}
Consider any function $\rho(W_1, W_2, \ldots, W_{\nu})$ where  $\rho :\{0,1\}^{\nu K} \rightarrow S$ for some set $S$. Then 
$$E\bigg[E\big[ |\{(w_1, w_2,\ldots w_{\nu}): \rho(w_1, w_2,\ldots w_{\nu}) = \rho(W_1, W_2,\ldots W_{\nu})\}| | W_1, W_2 \ldots W_{\nu} \big]\bigg] \geq 2^{\nu k-\log_{2}|S|}$$
\end{lemma}


Let $\mathcal{N}:\{0,1\}^{\nu K} \rightarrow \mathcal{P}(\{0,1\}^{K}$ be a set-valued function as follows:
$\mathcal{N}(W_1, W_2, \ldots, W_{\nu}) = \{\vec{x}: W_{1}, W_{2},\ldots, W_{\nu} \in \mathcal{B}(\vec{x},(\nu-1)\delta_{K}K)\}$ 

Note that $W_{i} \in \mathcal{N}(W_1, W_2, \ldots, W_{\nu})$ for all $i \in [\nu].$ Our main goal will be to show that 
\begin{itemize}
\item From every set of $c$ servers in the system, in every state with a common version among the servers, a decoder can recover at least one element of $\mathcal{N}(W_1, W_2, \ldots, W_{\nu}),$ and 
\item There exists a state such that, 
\end{itemize}


In this section, we briefly summarize the idea of the proof for $\nu=2$.
\begin{proof}[Proof of Theorem \ref{Theorem 5}]
	Consider any $\epsilon_K$-error $(n, c, \nu=2, 2^K, q)$ multi-version code, and consider the first $c \leq n$ servers $T=[c]$ for the converse. Suppose we have two versions $\mathbf W_{[2]}=(\mathbf W_1, \mathbf W_2)$. We partition the set of possible tuples $A_{\delta_K}$ as follows
	\begin{align}
	A_{\delta_K}= A_{\delta_K, 1} \cup A_{\delta_K, 2},
	\end{align}	
	where $A_{\delta_K, 1}$ is the set of all tuples $(\mathbf{w}_1, \mathbf{w}_2) \in A_{\delta_K}$ for which we can decode the latest common version or a later version successfully for all $\mathbf S  \in \mathcal{P}([\nu])^n$. $A_{\delta_K, 2}$ is the set of tuples where we cannot decode successfully at least for one state $\mathbf S  \in \mathcal{P}([\nu])^n$, which can be expressed as follows   
	\begin{align}
	A_{\delta_K, 2}= \bigcup_{\mathbf{S} \in \mathcal{P}([\nu])^n} A_{\delta_K, 2}^{(\mathbf S)},
	\end{align}
	where  $A_{\delta_K, 2}^{(\mathbf S)}$ is the set of tuples for which we cannot decode successfully given a state particular $\mathbf S \in \mathcal{P}([\nu])^n$. Consequently, we have
	\begin{align}
	|A_{\delta_K, 2}| \leq \sum_{\mathbf S \in \mathcal{P}([\nu])^n} |A_{\delta_K, 2}^{(\mathbf S)}|.
	\end{align}   
	For any state $\mathbf S \in \mathcal{P}([\nu])^n$, we require that 
	$P_e(\mathbf{S}, T) < \epsilon_K.$
	Since all tuples in the set $A_{\delta_K}$ are equiprobable, we have  
	\begin{align}
	P_e(\mathbf{S}, T)=\frac{|A_{\delta_K, 2}^{(\mathbf S)}|}{|A_{\delta_K}|},
	\end{align}	\color{black}
	consequently,  we have 
	
	\begin{align}
	|A_{\delta_K, 1}|&=|A_{\delta_K}|-|A_{\delta_K, 2}| \notag \\
	& \geq  |A_{\delta_K}|-\sum_{\mathbf S \in \mathcal{P}([\nu])^n} |A_{\delta_K, 2}^{(\mathbf S)}| \notag \\
	& > |A_{\delta_K}|-\sum_{\mathbf S \in \mathcal{P}([\nu])^n}  \epsilon_K  |A_{\delta_K}| \notag \\
	& >   |A_{\delta_K}|(1-\epsilon_K  2^{\nu n} ).
	\end{align}   
	Suppose that $(\mathbf W_1, \mathbf W_2) \in A_{\delta_K, 1}.$  \color{black}Because of the decoding requirements, if $\mathbf W_1$ is available at all servers, then the decoder must be able to obtain $\mathbf W_1$, and if $\mathbf W_2$ is available at all servers, then the decoder must return $\mathbf W_2$. Therefore, there must be two states $\mathbf{S}_1, \mathbf{S}_2 \in \mathcal{P}([\nu])^n$ such that
	\begin{itemize}
		\item $\mathbf{S}_1$ and $\mathbf{S}_2$ differ only in the state of one server indexed by $B \in [c]$.
		\item $\mathbf W_1$ can be recovered from the first $c$ servers in state $\mathbf{S}_1$ and $\mathbf W_2$ can be recovered from the first $c$ servers in $\mathbf{S}_2$.
	\end{itemize}
	Therefore both $\mathbf W_1$ and $\mathbf W_2$ are decodable from the $c$ codeword symbols of the first $c$ servers in state $\mathbf{S}_1$, and the codeword symbol of the $B$-th server in state $\mathbf{S}_2$. Thus, we require the following
	\begin{align*}
	c \ q^{c+1} &\geq |A_{\delta_K, 1}| \\
	& > |A_{\delta_K}|(1-\epsilon_K  2^{\nu n} )
	\end{align*}
	Because $\mathbf{W}_{1}$ is uniformly distributed in the set of all $K$ length binary vectors and given $\mathbf W_{1}$, $\mathbf W_{2}$ is uniformly distributed in a Hamming ball of radius $\delta_K K$ centered around $\mathbf W_1$, then we have
	\begin{align*}
	|A_{\delta_K}| = 2^K Vol(\delta_K K, K). \\
	\end{align*}
	In this case, the storage cost can be lower-bounded as follows
	\begin{align}
	\log q  \geq \frac{K+ \log  Vol(\delta_K K, K)}{c+1}+\frac{\log (1-\epsilon_K  2^{\nu n} )-\log c}{c+1}.    
	\end{align}
	%	Moreover, for $\delta_K=\delta$ where $\delta$ is a constant that is no larger than $1/2$, we have
	%	\begin{align}
	%	\mu=\frac{\log_2 q}{K}  \geq \frac{1+H(\delta)}{c+1}-\frac{\log_2 c+o(K)}{(c+1)K}.    
	%	\end{align}
	
\end{proof}

The lower bound in Corollary \ref{lower bound on binomial} follows since
\begin{align*}
Vol (\delta_K K, K)=\sum\limits_{j=0}^{\delta_K K}  \binom{K}{j} &\geq \binom{K}{\delta_K K}  \\ 
&= \prod_{i=0}^{\delta_K K-1} \frac{K-i}{\delta_K K-i} \\
&\geq \left(  \frac{1}{\delta_K } \right) ^{\delta_K K}.
\end{align*}

%\noindent  Finally, the bound in Corollary \ref{lower bound for constant delta} follows from Stirling's inequality \cite{feller1968introduction}. 


%In effect, this lower bound implies that the storage cost of any coding scheme is at least $\frac{K+(\nu-1) \log_2 Vol (K, \delta_K K)}{(c+\nu-1)K} - o(1).$ 
%If $\nu < c$, then storage cost attained by Theorem \ref{Theorem 3} is no larger than twice the lower bound, and therefore is order-optimal. 
\color{black}

